TAMS: Translation-Assisted Morphological Segmentation

Canonical morphological segmentation is the process of analyzing words into the standard (aka underlying) forms of their constituent morphemes. This is a core task in language documentation, and NLP systems have the potential to dramatically speed up this process. But in typical language documentation settings, training data for canonical morpheme segmentation is scarce, making it difficult to train high quality models. However, translation data is often much more abundant, and, in this work, we present a method that attempts to leverage this data in the canonical segmentation task. We propose a character-level sequence-to-sequence model that incorporates representations of translations obtained from pretrained high-resource monolingual language models as an additional signal. Our model outperforms the baseline in a super-low resource setting but yields mixed results on training splits with more data. While further work is needed to make translations useful in higher-resource settings, our model shows promise in severely resource-constrained settings.

==> modelsOrig.tex <==
\subsection{Model and Hyperparameters}

\label{subsec:hyperparam}
In preliminary experiments, we conduct a hyperparameter search with our models in order to find which model architectures, model sizes, and optimization methods are most effective for these datasets.
As it would be prohibitively expensive to do this in every experimental setting, we limit the scope of this search to baseline models (i.e., those that do not make any use of translation information) on the Tsez datasets on three training split sizes: 100, 500, and 6572.
The architectures we consider are the Transformer, the Pointer-Generator LSTM, and the Attentive LSTM.
Details are outlined in Appendix \ref{sec:appendixb}.

Regarding architecture, the pointer-generator LSTM \cite{see-etal-2017-get} performed better in all settings than either of the two other model architectures, and we therefore adopted it as our model architecture in all subsequent experiments.
Moreover, this choice is supported by evidence from \citet{Mager_Çetinoğlu_Kann_2020} that the pointer-generator is well suited to the low-resource canonical segmentation task. 

The pointer-generator LSTM differs from a regular LSTM encoder-decoder in that it has a pointer network \cite{Vinyals_Fortunato_Jaitly_2015}, which allows the model to copy over specific characters in the input sequence to the output sequence.
%It is a sequence-to-sequence model that combines and LSTM with a pointer network .  We model our implementation after \citet{see-etal-2017-get}
The decoder assesses the probability of copying an element from the input to the output rather than generating it, then computes the probability distribution of the output at each time step by combining the probability distribution across the output vocabulary with the attention distribution over the input characters. 
The weights, indicating the probability of generation or copying, are determined by a feedforward network. 

As for other hyperparameters, the results of our search are not significantly different for the two larger settings but vary notably for the 100-sample training split setting. 
As such, in all subsequent experiments, we train our 100 training sample models with one set of hyperparameters and all other models with a separate set. 
Both settings use the Adam optimizer and the ReduceLROnPlateau scheduler.

%We conduct a hyperparameter search on a range of hyperparameters affecting model architecture, model size, and optimization.  As it would be prohibitively expensive to conduct a hyperparameter search for each possible combination language and translation incorporation strategy, we limit our search to Tsez baseline models at each train-data setting. In order to determine whether training split size influences a model's optimal hyperparameters, we conduct our hyperparameter search with three different training split sizes: 100, 500, and 6572. 

For experimental settings 100 training samples, use a batch size of 16, two encoder and two decoder layers, an embedding size of 512 and a hidden size of 1024. 
We set dropout to $3.662 \times 10^{-1}$, learning rate to $2.411 \times 10^{-4}$, and train for a maximum of 607 epochs.

For all other experimental settings, we use a batch size of 64, one encoder and one decoder layer, an embedding size of 1024, and a hidden size of 2048. 
We set dropout to $2.212 \times 10^{-1}$, learning rate to $8.056 \times 10^{-4}$, and train for a maximum of 627 epochs. 

% \subsection{Baseline}
% We compare our models to a baseline pointer-generator LSTM trained with same set of hyperparameters that does not employ any translation incorporation strategies.

\subsection{Optimal Translation Incorporation Configuration}

We treat translation incorporation strategy as a hyperparameter and test all possible pairings of strategies on the Tsez development set to determine the optimal approach. We take the average whole-word accuracy for configuration across all training split sizes on the Tsez development set using the \textbf{CLS-None} strategy. The full results of this search are shown in Table \ref{table:mega-tsez}. From this search, we find that the overall highest performing strategy configuration is \textbf{Init-State} in the encoder and \textbf{Concat-Half} in the decoder. This configuration outperforms the baseline by an average of 1.58\% and is the top performer on the 100 and 500 train sample settings. Only in the highest train data setting does the baseline outperform our top configuration. For the 100 train sample setting, \textbf{Concat} in the encoder and \textbf{Concat-Half} in the decoder, the second highest performing configuration overall, was the top configuration. With this in mind, we perform a second search over the CLS strategies on these two configurations, shown in Table \ref{table:Cls-tsez}.  From this, we find that the overall highest performing configuration is \textbf{Init-State} in the encoder, \textbf{Concat-Half} in the decoder and \textbf{CLS-Concat} as our CLS Strategy; we call this model \textbf{TAMS}.

==> old_abstract.tex <==
Canonical morphological segmentation is the process of splitting words into the standard forms of their composite morphemes.
The task is a vital component of language documentation work, 
but canonical segmentation data can be hard to come by.
However, in the documentation setting, translation data is often more abundant and/or easier to obtain.
In this paper, we investigate a novel approach to neural canonical segmentation that leverages this underutilized data source.
We train a sequence-to-sequence LSTM model that incorporates translations as an additional signal in the form of BERT embeddings.
RESULTS
